A dynamic programming algorithm for span-based nested named-entity recognition in O(n^2)

Span-based nested named-entity recognition (NER) has a cubic-time complexity using a variant of the CYK algorithm. We show that by adding a supplementary structural constraint on the search space, nested NER has a quadratic-time complexity, that is the same asymptotic complexity than the non-nested case. The proposed algorithm covers a large part of three standard English benchmarks and delivers comparable experimental results.

==> floats/ablation.tex <==


\begin{table*}[]
    \centering
    \small
    
    % new results
    % /mnt/beegfs/home/corro/interpretable-nn/ner/exp/2022-06-20_00:54:05.905639
    % on garde seulement CRF et CRF + smoothing
    \begin{tabular}{@{}ll@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{}}
        \toprule
         && \multicolumn{9}{c}{Dataset} \\
         \cmidrule{3-11}
         && \multicolumn{3}{c}{\textsc{Ace-2004}} & \multicolumn{3}{c}{\textsc{Ace-2005}} & \multicolumn{3}{c}{\textsc{Genia}} \\
         && Prec. & Rec. & F1 & Prec. & Rec. & F1 & Prec. & Rec. & F1 \\
         %\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
         \midrule
         \textsc{Crf} loss  & CYK-like
         & 87.18 & 86.06 & 86.62 % ACE 2004
         & 83.39 & 85.51 & 84.44  % ACE 2005
         & 77.33 & 78.13 & 77.72  % Genia
         \\
         & Proposed alg.
          & 87.37 & 85.04 & 86.19  % ACE 2004
         & 83.75 & 85.25 & 84.49  % ACE 2005
         & 77.46 & 77.98 & 77.72 % Genia
         \\
         \midrule
         + smoothing 0.01 & CYK-like 
          &86.15 & 86.92 & 86.53  % ACE 2004
         & 83.72 & 86.24 & 84.96  % ACE 2005
         & 78.26 & 77.57 & 77.91 % Genia
         \\
         & Proposed alg.
          & 86.34 & 85.83 & 86.09  % ACE 2004
         & 84.02 & 85.74 & 84.87  % ACE 2005
         & 78.39 & 77.48 & 77.94 % Genia
         \\
         \midrule
         + smoothing 0.05 & CYK-like 
          & 86.07 & 86.56 & 86.32  % ACE 2004
         & 84.47 & 86.34 & 85.39 % ACE 2005
         & 79.12 & 76.73 & 77.91 % Genia
         \\
         & Proposed alg.
          & 86.40 & 85.40 & 85.90  % ACE 2004
         & 84.53 & 85.64 & 85.08  % ACE 2005
         & 79.11 & 76.63 & 77.85 % Genia
         \\
         \midrule
         + smoothing 0.1 & CYK-like 
          & 86.54  & 86.43 & 86.48  % ACE 2004
         & 84.20 & 85.84 & 85.01 % ACE 2005
         & 79.20 & 77.31 & 78.24 % Genia
         \\
         & Proposed alg.
          & 86.79 & 85.30 & 86.04  % ACE 2004
         & 84.42 & 85.28 & 84.85  % ACE 2005
         & 79.28 & 77.25 & 78.25 % Genia
         \\
         \midrule
         + margin  & CYK-like
          & 86.29 & 86.10 & 86.19  % ACE 2004
         &  83.49 & 85.31 & 84.39  % ACE 2005
         & 80.86 & 74.59 & 77.60 % Genia
         \\
         & Proposed alg.
          & 86.57 & 84.98 & 85.77  % ACE 2004
         & 83.89 & 85.08 & 84.48  % ACE 2005
         & 80.88 & 74.55 & 77.59 % Genia
         \\
         \midrule
         + smoothing 0.01 + margin  & CYK-like 
          & 85.97      & 86.19 & 86.08  % ACE 2004
         &  83.26 & 85.84 & 84.53  % ACE 2005
         & 79.25 & 76.73 & 77.97 % Genia
         \\
         & Proposed alg. 
          & 86.03 & 85.04 & 85.53  % ACE 2004
         & 83.48 & 85.41 & 84.44 % ACE 2005
         & 79.27 & 76.66 & 77.94 % Genia
         \\
         \midrule
         + smoothing 0.05 + margin  & CYK-like 
          &86.22 & 86.00 & 86.11  % ACE 2004
         & 84.17 & 85.45 & 84.80  % ACE 2005
         & 78.06 & 77.93 & 77.99 % Genia
         \\
         & Proposed alg. 
          & 86.33 & 84.71 & 85.51  % ACE 2004
         & 84.32 & 84.98 & 84.65  % ACE 2005
         & 78.17 & 77.88 & 78.02 % Genia
         \\
         \midrule
         + smoothing 0.1 + margin  & CYK-like 
          & 86.81 & 86.33 & 86.57  % ACE 2004
         & 84.02 & 85.58 & 84.79  % ACE 2005
         &79.76 & 75.96 & 77.81 % Genia
         \\
         & Proposed alg. 
          & 87.04 & 85.17 & 86.09  % ACE 2004
         & 84.16 & 85.05 & 84.60  % ACE 2005
         & 79.82 & 75.96 & 77.84% Genia
         \\
         \bottomrule
    \end{tabular}
    \caption{Ablation results.}
    \label{tab:results}
\end{table*}



==> floats/ablation_max_len.tex <==

         \midrule
         \multicolumn{11}{l}{\textbf{With length constraint}} \\
         \midrule
         \textsc{Crf} loss  & CYK-like
         & 85.90 & 85.93 & 85.92 % ACE 2004
         & 82.35 & 86.07 & 84.17  % ACE 2005
         & 79.03 & 65.80 & 71.81  % Genia
         \\
         & Proposed alg.
         & 86.20 & 85.24 & 85.72 % ACE 2004
         & 82.89 & 85.68 & 84.26 % ACE 2005
         & 79.11 & 65.78 & 71.83  % Genia
         \\
         \midrule
         + smoothing  & CYK-like 
         & 85.65 & 85.57 & 85.61  % ACE 2004
         & 82.34 & 85.84 & 84.05  % ACE 2005
         & 76.14 & 69.57 & 72.71 % Genia
         \\
         & Proposed alg. 
         & 85.98 & 84.68 & 85.33  % ACE 2004
         & 82.65 & 85.21 & 83.91  % ACE 2005
         & 76.20 & 69.44 & 72.66  % Genia
         \\
         \midrule
         + margin  & CYK-like 
         & 86.30 & 85.11 & 85.70  % ACE 2004
         & 84.59 & 84.79 & 84.69 % ACE 2005
         & 76.47 & 69.53 & 72.84 % Genia
         \\
         & Proposed alg. 
         & 86.41 & 84.22 & 85.30 % ACE 2004
         & 84.97 & 84.49 & 84.73  % ACE 2005
         & 76.60 & 69.44 & 72.85  % Genia
         \\
         \midrule
         + pot. reg.  & CYK-like 
         & 86.59 & 84.05 & 85.30 % ACE 2004
         & 82.32 & 83.76 & 83.04 % ACE 2005
         & & &  % Genia
         \\
         & Proposed alg. 
         & 86.62 & 82.97 & 84.75 % ACE 2004
         & 82.65 & 83.47 & 83.05 % ACE 2005
         & & &  % Genia
         \\
         \midrule
         + smoothing + margin  & CYK-like 
         & 85.46 & 85.80 & 85.63 % ACE 2004
         & 82.92 & 85.21 & 84.05  % ACE 2005
         & 77.50 & 68.76 & 72.87 % Genia
         \\
         & Proposed alg. 
         & 85.81 & 84.68 & 85.24 % ACE 2004
         & 83.36 & 84.82 & 84.08 % ACE 2005
         & 77.59 & 68.73 & 72.89 % Genia
         \\
         \midrule
         + margin + pot. reg.  & CYK-like 
         & 86.26 & 84.38 & 85.31  % ACE 2004
         & 82.69 & 84.06 & 83.37 % ACE 2005
         & & &  % Genia
         \\
         & Proposed alg. 
         & 86.51 & 83.49 & 84.98 % ACE 2004
         & 83.01 & 83.53 & 83.27 % ACE 2005
         & & &  % Genia
         \\
         + smoothing + pot. reg.  & CYK-like
         & 85.40 & 85.93 & 85.66 % ACE 2004
         & 81.30 & 85.64 & 83.41 % ACE 2005
         & 66.22 & 68.46 & 67.32 % Genia
         \\
         & Proposed alg.
         & 86.04 & 84.88 & 85.45 % ACE 2004
         & 81.84 & 85.08 & 83.43 % ACE 2005
         & 68.15 & 68.50 & 68.32 % Genia
         \\
         \midrule
         + smoothing + margin + pot. reg.  & CYK-like 
         & & &  % ACE 2004
         & & &  % ACE 2005
         & & &  % Genia
         \\
         & Proposed alg. 
         & & &  % ACE 2004
         & & &  % ACE 2005
         & & &  % Genia
         \\

==> floats/ablation_no_lstm.tex <==
         \multicolumn{11}{l}{\textbf{No length constraint}} \\
         \midrule
         \textsc{Crf} loss  & CYK-like
         & 84.93 & 85.60 & 85.26 % ACE 2004
         &  82.20 & 84.92 & 83.54  % ACE 2005
         &  &  &  % Genia
         \\
         & Proposed alg.
         & 85.71 & 84.61 & 85.16 % ACE 2004
         &  82.81 & 84.55 & 83.67   % ACE 2005
         &  &  &  % Genia
         \\
         \midrule
         + smoothing 0.01 & CYK-like 
         & 84.67 & 85.73 & 85.20  % ACE 2004
         &  82.24 & 84.69 & 83.45   % ACE 2005
         &  &  &  % Genia
         \\
         & Proposed alg.
          & 85.25 & 84.71 & 84.98 % ACE 2004
         & 82.81 & 84.29 & 83.55   % ACE 2005
         &  &  &  % Genia
         \\
         \midrule
         + smoothing 0.05 & CYK-like 
          & 84.65 & 85.93 & 85.28  % ACE 2004
         &  82.45 & 85.12 & 83.76  % ACE 2005
         &  &  &  % Genia
         \\
         & Proposed alg.
          & 85.31 & 84.78 & 85.04  % ACE 2004
         & 82.99 & 84.55 & 83.77   % ACE 2005
         &  &  &  % Genia
         \\
         \midrule
         + smoothing 0.1 & CYK-like 
          & 84.94 & 85.67 & 85.30  % ACE 2004
         &  82.46 & 85.31 & 83.86   % ACE 2005
         &  &  &  % Genia
         \\
         & Proposed alg.
          & 85.51 & 84.61 & 85.06  % ACE 2004
         & 82.90 & 84.65 & 83.77    % ACE 2005
         &  &  &  % Genia
         \\
         \midrule
         + margin  & CYK-like
          & 84.61 & 85.34 & 84.97  % ACE 2004
         & 82.91 & 84.69 & 83.79 % ACE 2005
         &  &  &  % Genia
         \\
         & Proposed alg.
          & 85.16 & 84.35 & 84.75  % ACE 2004
         & 83.32 & 84.22 & 83.77   % ACE 2005
         &  &  &  % Genia
         \\
         \midrule
         + smoothing 0.01 + margin  & CYK-like 
          & 85.05 & 85.47 & 85.26  % ACE 2004
         &  & &   % ACE 2005
         &  &  &  % Genia
         \\
         & Proposed alg. 
          & 85.86 & 84.61 & 85.23  % ACE 2004
         &  & &   % ACE 2005
         &  &  &  % Genia
         \\
         \midrule
         + smoothing 0.05 + margin  & CYK-like 
          & 85.49 & 85.40 & 85.45  % ACE 2004
         &  & &   % ACE 2005
         &  &  &  % Genia
         \\
         & Proposed alg. 
          & 85.99 & 84.51 & 85.24  % ACE 2004
         &  & &   % ACE 2005
         &  &  &  % Genia
         \\
         \midrule
         + smoothing 0.1 + margin  & CYK-like 
          & 85.26 & 86.13 & 85.69  % ACE 2004
         & 82.86  & 84.88 & 83.8  % ACE 2005
         &  &  &  % Genia
         \\
         & Proposed alg. 
          & 85.87 & 85.07 & 85.47  % ACE 2004
         & 83.41 & 84.29 & 83.85 % ACE 2005
         &  &  &  % Genia
         \\
         \midrule
         LSTM 3 \\

==> floats/ablation_old.tex <==
\begin{table*}[]
    \centering
    \small
    \begin{tabular}{@{}ll@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{}}
        \toprule
         && \multicolumn{9}{c}{Dataset} \\
         \cmidrule{3-11}
         && \multicolumn{3}{c}{\textsc{Ace-2004}} & \multicolumn{3}{c}{\textsc{Ace-2005}} & \multicolumn{3}{c}{\textsc{Genia}} \\
         && Prec. & Rec. & F1 & Prec. & Rec. & F1 & Prec. & Rec. & F1 \\
         %\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
         \midrule
         \multicolumn{11}{l}{\textbf{No length constraint}} \\
         \midrule
         \textsc{Crf} loss  & CYK-like
         & 85.17 & 86.49 & 85.83 % ACE 2004
         & 82.80 &85.18 & 83.98  % ACE 2005
         & 77.69 & 73.78 & 75.69 % Genia
         \\
         & Proposed alg.
         & 85.84 & 85.50 & 85.67  % ACE 2004
         & 83.06 & 84.79 & 83.91 % ACE 2005
         & 77.78 & 73.73 & 75.70 % Genia
         \\
         \midrule
         + smoothing  & CYK-like 
         & 85.40 & 86.13 & 85.76 % ACE 2004
         & 83.58 & 85.51 & 84.54 % ACE 2005
         & 76.04 & 75.43 & 75.73  % Genia
         \\
         & Proposed alg.
         & 85.54 & 84.98 & 85.26 % ACE 2004
         & 84.01 & 84.82 & 84.41   % ACE 2005
         & 76.08 & 75.36 & 75.72 % Genia
         \\
         \midrule
         + margin  & CYK-like
         & 86.24 & 84.91 & 85.57  % ACE 2004
         & 83.23 & 85.02 & 84.11  % ACE 2005
         & 77.82 & 73.55 & 75.63 % Genia
         \\
         & Proposed alg.
         & 86.54 & 84.12 & 85.31  % ACE 2004
         & 83.45 & 84.52 & 83.98  % ACE 2005
         & 77.93 & 73.46 & 75.63  % Genia
         \\
         %\midrule
         %+ pot. reg.  & CYK-like 
         %& 84.59 & 86.43 & 85.50 % ACE 2004
         %& 85.33 & 82.54 & 83.91 % ACE 2005
         %& 77.50 & 71.09 & 74.15 % Genia
         %\\
         %& Proposed alg. 
         %& 85.00 & 85.30 & 85.15 % ACE 2004
         %& 85.50 & 82.34 & 83.89 % ACE 2005
         %& 77.64 & 71.03 & 74.19  % Genia
         %\\
         \midrule
         + smoothing + margin  & CYK-like 
         & 86.10 & 85.73 & 85.92  % ACE 2004
         & 83.67 & 85.74 & 84.69 % ACE 2005
         & 77.41 & 75.09 & 76.23  % Genia
         \\
         & Proposed alg. 
         & 86.37 & 84.55 & 85.45  % ACE 2004
         & 83.82 & 85.15 & 84.48  % ACE 2005
         & 77.45 & 74.98 & 76.19  % Genia
         \\
         %\midrule
         %+ margin + pot. reg.  & CYK-like 
         %& 84.79 & 84.48 & 84.63 % ACE 2004
         %& 82.79 & 84.92 & 83.84 % ACE 2005
         %& 78.38 & 72.32 & 75.23 % Genia
         %\\
         %& Proposed alg.
         %& 85.15 & 83.69 & 84.41  % ACE 2004
         %& 83.30 & 84.62 & 83.96 % ACE 2005
         %& 78.47 & 72.30 & 75.26 % Genia
         %\\
         %\midrule
         %+ smoothing + pot. reg.  & CYK-like
         %& 85.90 & 84.68 & 85.28 % ACE 2004
         %& 82.78 & 85.51 & 84.12  % ACE 2005
         %& 78.01 & 72.46 & 75.13 % Genia
         %\\
         %& Proposed alg.
         %& 86.26 & 83.79 & 85.01 % ACE 2004
         %& 83.04 & 84.85 & 83.94 % ACE 2005
         %& 78.01 & 72.41 & 75.11 % Genia
         %\\
         %\midrule
         % Warning, this is
         % + smoothing + margin + pot. reg. 
         % but the last op is on the prev line
         %+ smoothing + margin   & CYK-like
         %& 86.42 & 85.54 & 85.97 % ACE 2004
         %& 83.88 & 85.51 & 84.69 % ACE 2005
         %& 77.68 & 72.89 & 75.21 % Genia
         %\\
         %+ pot. reg. & Proposed alg.
         %& 86.78 & 84.55 & 85.65  % ACE 2004
         %& 84.07 & 85.02 & 84.54 % ACE 2005
         %& 77.74 & 72.84 & 75.21  % Genia
         %\\
         \bottomrule
    \end{tabular}
    
    \caption{Ablation results.}
    \label{tab:results}
\end{table*}


==> floats/results_bis.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{@{}l@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{}}
        \toprule
         & \multicolumn{9}{c}{Dataset} \\
         \cmidrule{2-10}
         & \multicolumn{3}{c}{\textsc{Ace-2004}} & \multicolumn{3}{c}{\textsc{Ace-2005}} & \multicolumn{3}{c}{\textsc{Genia}} \\
         & Prec. & Rec. & F1 & Prec. & Rec. & F1 & Prec. & Rec. & F1 \\
         %\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
         \midrule
         \multicolumn{10}{l}{\textbf{Comparable models based on BERT}} \\
         \midrule
         %
         \citet{shibuya2020secondbest} & 85.23 & 84.72 & 84.97 & 83.30 & 84.69 & 83.99 & 77.46 & 76.65 & 77.05\\
         %+ Flair & 85.94 & 85.69 & 85.82 & 83.83 & 84.87 & 84.34 & 77.81 & 76.94 & 77.36 \\
         %
         \citet{wang2020pyramid} & 86.08 & 86.48 & 86.28 & 83.95 & 85.39 & 84.66 & 79.45 & 78.94 & 79.19 \\
         % + autres expés avec Flair, Alberta, combinaison erc
         %
         \citet[][max]{wang2021excludesecondbest} & 86.27 & 85.09 & 85.68 & 85.28 & 84.15 & 84.71 &  79.20 & 78.16 & 78.67\\
         %
         \citet{fu2021latentcyk}\textsuperscript{\textdagger} & 87.62 & 87.57 & 87.60 & 83.34 & 85.67 & 84.49 & 79.10 & 76.53 & 77.80 \\
         \citet{tan2021seqtoset}\textsuperscript{\textdagger} & 87.05 & 86.26 & 86.65 & 83.92 & 84.75 & 84.33 & 78.33 & 76.66 & 77.48 \\
         \citet{shen2021locate}\textsuperscript{\textdagger} & 87.27 & 86.61 & 86.94 & 86.02 & 85.62 & 85.82 & 76.80 & 79.02 & 77.89 \\
         \citet{yan2021unifiedgen} & 87.27 & 86.41 & 86.84 & 83.16 & 86.38 & 84.74 & 78.57 & 79.3 & 78.93 \\
         \midrule
         \multicolumn{10}{l}{\textbf{This work}} \\
         \midrule
% /mnt/beegfs/home/corro/interpretable-nn/ner/exp/2022-06-20_00:54:05.905639
% on garde seulement CRF et CRF + smoothing 0.1
         Semi-Markov algorithm, $\mathcal O(n^2)$
%
         CYK-like algorithm, $\mathcal O(n^3)$ 
          & 87.18 & 86.06 & 86.62 % ACE 2004
         & 83.39 & 85.51 & 84.44  % ACE 2005
         & 77.33 & 78.13 & 77.72  % Genia
         \\
%
         + smoothing 
       & 86.54  & 86.43 & 86.48  % ACE 2004
         & 84.20 & 85.84 & 85.01 % ACE 2005
         & 79.20 & 77.31 & 78.24 % Genia
         \\
%
         Proposed algorithm, $\mathcal O(n^2)$ 
                   & 87.37 & 85.04 & 86.19  % ACE 2004
         & 83.75 & 85.25 & 84.49  % ACE 2005
         & 77.46 & 77.98 & 77.72 % Genia
         \\
%
         + smoothing
                   & 86.79 & 85.30 & 86.04  % ACE 2004
         & 84.42 & 85.28 & 84.85  % ACE 2005
         & 79.28 & 77.25 & 78.25 % Genia
         \\
         \midrule
         \multicolumn{10}{l}{\textbf{Other works}} \\
         \midrule
         \citet{lou2022latentlex} & 87.39 & 88.40 & 87.90 & 85.97 & 87.87 & 86.91 & 78.39 & 78.50 & 78.44 \\
         \bottomrule
    \end{tabular}
    \caption{Precision, recall and F1-measure results. We compare ourselves to other BERT-based models --- some of the cited papers includes richer models that we omit for brievity as our goal is only to asses the performance of our algorithm compared to the CYK-like one. Results marked with \textdagger are the reproduction of \cite{lou2022latentlex} as the original papers experimented on different data splits.}
    \label{tab:results}
\end{table*}


==> training.tex <==
\section{Training with latent alignment}

A dataset $E = \{(w_i, z_i)\}_{i=1}^M$ is composed of $M$ tuples where $w_i$ is a natural language utterance and $z_i$ is the corresponding program.
During training, we want to learn to map the utterance $w_i$ to a semantic tree that will produce the program $z_i$.
That is, we want our model to learn to maximize the likelihood of the correct tree.

\paragraph{Computing the likelihood of a tree} For a given sentence of length $N$, to compute the likelihood of a tree, we first need to define the set of all possible trees.
We saw earlier that a tree could be represented by two vectors $\vx$ and $\vy$.
We write $\mathcal{X}$ the set of all possible values that the vector $\vx$ can take which are all the combinations such that exactly one vertex is selected in every cluster. More formally, it is written as :
\[ \mathcal{X} = \{ x \in [0,1]^{|V|} | \forall i \in \{0, 1, ..., n\} : \sum_{v \in V_i} x_v = 1 \} \]
Similarly, we define $\mathcal{Y}$ as the set of all possible selections of arcs that result in a generalized spanning arborescence.
The subset $\mathcal{Y}(\vx)$ represent the possible values of $\vy$ for a given $\vx$ such that the tree is valid with respect to the semantic language.
We define $X \in \mathcal{X}$ a random variable that represents the selection of one node per cluster.
$Y \in \mathcal{Y}$ is the selection of a set of arcs that form a generalized spanning arborescence.
The joint probability of the two random variables $X$ and $Y$ can be defined as :
\[ P(X=x, Y=y) = exp(s(x,y) - Z) \]
where we assume that $exp(-\infty) = 0$. 
$s(x,y)$ is equal to $\mu^\top \vx + \phi^\top \vy$ if $y \in \mathcal{Y}(x)$ and $-\infty$ otherwise. 
The value $Z = log \sum_{x' \in \mathcal{X}} \sum_{y' \in \mathcal{Y}(x)} exp(s(x',y'))$ is the log-partition function that normalizes the distribution. 

\paragraph{Latent alignment} The dataset does not contain the alignment between the words in a sentence $w_i$ and the various predicates that form the associated program $z_i$.



\begin{align*}
	p(\vx, \vy)
	= \exp(\phi^\top \vx + \mu^\top \vy - c(\phi, \mu))
\end{align*}
where $c(\phi, \mu) = \log \sum_{\vx'} \sum_{\vy'} \exp(\phi^\top \vx' + \mu^\top \vy')$ is the log-partition function.

\begin{align*}
\log \sum_{\vx, \vy} p(\vx, \vy)
&= \log \sum_{\vx, \vy} \frac{\exp(\phi^\top \vx + \mu^\top \vy)}{Z} \\
&\hspace{-2cm}=\log \left (\sum_{\vx, \vy} \exp(\phi^\top \vx + \mu^\top \vy) \right) - \log Z
\end{align*}

Unfortunately, none of these terms is tractable.


\subsection{Partition function}

\begin{align*}
c(\phi, \mu)
&= \max_{\vp} \vp ^\top \nu + \entropy(\vp) \\
\intertext{where $H$ is the entropy function defined as $H(\vp) = -\sum_i \evp_i \log \evp_y$.}
&= \max_{(\vx, \vy) \in \marginal} \vu ^\top \nu + \entropy_{\marginal}(\vx, \vy)
\intertext{%
Where $\conv(\feasible)$ is the marginal polytope and $H_{\conv(\feasible)}$ is the function defined such that: TODO.
Unfortunately, this optimization is hard to solve as $\marginal$ cannot be characterized in an explicit manner and the exact entropy $\entropy_{\marginal}(\vx, \vy)$ is defined indirectly and lacks a polynomial closed form solution \cite[Section 3.7]{wainwright2008exp}.
However, we can approximate the true log-partition function by using an outer bound to the marginal polytope $\relmarginal \supset \marginal$ and approximating the exact entropy regularizer $\entropy_{\marginal}$ with mean parameter regularization:
}
&\simeq \max_{(\vx, \vy) \in \relmarginal} \vx ^\top \phi + \vx ^\top \mu + \entropy(\vx) +\entropy(\vy) \\
&=\tilde{c}(\phi, \mu)
\end{align*}
For training, we need to compute the gradient of the (approximate) log partition function $\nabla_{(\phi, \mu)} \tilde{c}(\phi, \mu)$.
As $\tilde{c}(\phi, \mu)$ is defined as the maximum of a strictly concave function, the maximizer is unique and therefore, by Danskin's theorem \cite{danskin1966theory}:
$$
	\nabla_{(\phi, \mu)} \tilde{c}(\phi, \mu) = \stacktwo{\vx}{\vy},
$$
i.e.\ the gradient wrt to the distribution parameters is the mean parameters.


\subsection{Latent alignment}

$$
c(S, \phi, \mu) = \log \sum_{\vx, \vy \in S} \exp(\phi^\top \vx + \mu^\top \vy)
$$
